Flexible Diffusion Scopes with Parameterized Laplacian for Heterophilic Graph Learning

The ability of Graph Neural Networks (GNNs) to capture long-range and global topology information is limited by the scope of conventional graph Laplacian, leading to unsatisfactory performance on some datasets, particularly on heterophilic graphs. To address this limitation, we propose a new class of parameterized Laplacian matrices, which provably offers more flexibility in controlling the diffusion distance between nodes than the conventional graph Laplacian, allowing long-range information to be adaptively captured through diffusion on graph. Specifically, we first prove that the diffusion distance and spectral distance on graph have an order-preserving relationship. With this result, we demonstrate that the parameterized Laplacian can accelerate the diffusion of long-range information, and the parameters in the Laplacian enable flexibility of the diffusion scopes. Based on the theoretical results, we propose topology-guided rewiring mechanism to capture helpful long-range neighborhood information for heterophilic graphs. With this mechanism and the new Laplacian, we propose two GNNs with flexible diffusion scopes: namely the Parameterized Diffusion based Graph Convolutional Networks (PD-GCN) and Graph Attention Networks (PD-GAT). Synthetic experiments reveal the high correlations between the parameters of the new Laplacian and the performance of parameterized GNNs under various graph homophily levels, which verifies that our new proposed GNNs indeed have the ability to adjust the parameters to adaptively capture the global information for different levels of heterophilic graphs. They also outperform the state-of-the-art (SOTA) models on 6 out of 7 real-world benchmark datasets, which further confirms their superiority.

==> table_dataset.tex <==
\begin{table}[htbp]
  \centering  
  \begin{tabular}{c|ccccccccc}
  \toprule
  \toprule
    & Cham.
    & Squi.
    & Actor
    & Corn. 
    & Wisc. 
    & Texas  
    & Cora  
    & Cite.
    & Pubm.  \\
    
    \midrule
    \# Nodes 
    & 2,277
    & 5,201
    & 7,600
    & 183   
    & 251   
    & 183  
    & 2,708 
    & 3,327 
    & 19,717 \\
    
    \# Edges 
    & 36,101
    & 217,073
    & 33,544
    & 295   
    & 499   
    & 309  
    & 5,429 
    & 4,732 
    & 44,324 \\
    
    \# Features 
    & 2,325
    & 2,089
    & 931
    & 1,703 
    & 1,703 
    & 1,703 
    & 1,433 
    & 3,703
    & 500 \\
    
    \# Classes 
    & 5
    & 5
    & 5
    & 5     
    & 5     
    & 5    
    & 7     
    & 6
    & 3 \\
    
    $H_{\mathrm{node}}(G)^{\star}$
    & 0.23
    & 0.22
    & 0.22
    & 0.30
    & 0.21
    & 0.11
    & 0.81
    & 0.74
    & 0.80 \\
    
  \bottomrule
  \bottomrule
  \end{tabular}
  \caption{Benchmark dataset statistics. The $\star$ statistics are reported from \cite{ma2021homophily}.}
    
\end{table}


==> table_hyperparameters.tex <==
\begin{table}[h!]
 \resizebox{1\hsize}{!}{
  \begin{tabular}{lcccccc}
  \toprule

    Dataset ($\mathbf{H}_{\mathrm{node}}(\mathcal{G})$) &
    % Models\textbackslash{}Hyperparameters &
    learning rate &
    weight decay &
    dropout &
    $\epsilon$  &
    $\gamma$ &
    $\alpha$
    \\

    \midrule
    chameleon (0.25)&
    $5 \times 10^{-3}$ & 
    $5 \times 10^{-4}$ &
    0.4 &
    % $5 \times 10^{-6}$ &
    $1 \times 10^{-7}$ &
    0.0 &
    0.9
    \\
    
    %\midrule
    squirrel (0.22)&
    $5 \times 10^{-2}$ & 
    $5 \times 10^{-5}$ &
    % 0.5 &
    % $5 \times 10^{-6}$ &
    0.2 &
    $1 \times 10^{-7}$ &
    0.2 &
    0.1
    \\

    %\midrule
    actor (0.22)&
    $1 \times 10^{-5}$ & 
    $1 \times 10^{-7}$ &
    % 0.2 &
    % $5 \times 10^{-4}$ &
    0.3 &
    $1 \times 10^{-7}$ &
    0.2 &
    0.2 
    \\
    
    %\midrule
    cornell (0.30) &
    $5 \times 10^{-3}$ & 
    $5 \times 10^{-4}$ &
    0.2 &
    $5 \times 10^{-6}$ &
    0.3 &
    0.8
    \\
    
    %\midrule
    wisconsin (0.16) &
    $5 \times 10^{-3}$ & 
    $5 \times 10^{-6}$ &
    % 0.2 &
    % $5 \times 10^{-6}$ &
    0.5 &
    $1 \times 10^{-6}$ &
    0.3 &
    0.7
    \\
    
    %\midrule
    texas (0.06) &
    $5 \times 10^{-5}$ & 
    $5 \times 10^{-3}$ &
    % 0.4 &
    % $5 \times 10^{-3}$&
    0.4 &
    $1 \times 10^{-5}$&
    0.2 &
    0.8 
    \\
    
    %\midrule
    cora (0.83) &
    $5 \times 10^{-3}$ & 
    $5 \times 10^{-4}$ &
    % 0.5 &
    % $ 1\times 10^{-5}$&
    0.4 &
    $ 5\times 10^{-7}$&
    0.9 &
    0.8 
    \\
    
    %\midrule
    citeseer (0.71)&
    $5 \times 10^{-2}$ & 
    $5 \times 10^{-5}$ &
    % 0.3 &
    0.6 &
    $ 1\times 10^{-5}$&
    0.5 &
    0.2 
    \\
    
    %\midrule
    % {\textbf{PubMed}}
    pubmed (0.79) &
    $1 \times 10^{-2}$ & 
    $5 \times 10^{-2}$ &
    % 0.5 &
    % $ 1\times 10^{-5}$&
    0.6 &
    $ 1\times 10^{-6}$ &
    1 &
    0.3
    \\

    
  \bottomrule
  \end{tabular}
  }
  \caption{Hyperparameters of DGAT on geom datasets}
  \label{table:hyper}
    
\end{table}

==> table_result.tex <==
%\begin{table}[htbp]
\begin{table}[t]
  \centering  
%   \tiny
%   \setlength{\tabcolsep}{0.5pt}
  \begin{tabular}{c|ccccccccc}
  \toprule
  \toprule
    & Cham.
    & Squi.
    & Actor
    & Corn. 
    & Wisc. 
    & Texas  
    & Cora  
    & Cite.
    & Pubm.  \\
    
    \midrule
    
    $\text{GAT}^{\dag}$  &
    42.93 &
    30.03 &
    28.45 & 
    54.32 & 
    49.41 & 
    58.38 & 
    86.37 &
    74.32 &
    87.62  \\
    
    $\text{DGN}^{\ddag}$  &
    50.48 &
    \cellcolor[rgb]{ .816,  .808,  .808}\textbf{37.46} &
    35.47 & 
    77.03 & 
    82.75 & 
    78.11 & 
    84.69 &
    73.87 &
    84.29  \\
    
    DGAT & 
    \cellcolor[rgb]{ .816,  .808,  .808}\textbf{52.47} &
    34.82 &
    \cellcolor[rgb]{ .816,  .808,  
    .808}\textbf{35.68} &
    \cellcolor[rgb]{ .816,  .808,  
    .808}\textbf{85.14} & 
    \cellcolor[rgb]{ .816,  .808,  
    .808}\textbf{84.71} & 
    \cellcolor[rgb]{ .816,  .808,  
    .808}\textbf{79.46} & 
    \cellcolor[rgb]{ .816,  .808,  .808}\textbf{88.05} & 
    \cellcolor[rgb]{ .816,  .808,  .808}\textbf{76.41}  &
    \cellcolor[rgb]{ .816,  .808,  .808}\textbf{87.93}
    \\
    
    \midrule
    $H_{\mathrm{node}}(\mathcal{G})$
    & 0.23
    & 0.22
    & 0.22
    & 0.30
    & 0.21
    & 0.11
    & 0.81
    & 0.74
    & 0.80 \\

  \bottomrule
  \bottomrule
  \end{tabular}
  \caption{Experimental results: average test accuracy (\%) of 9 real-world benchmark datasets. 
  The best results are highlighted. 
  Results "$\dag$" are reported from \cite{pei2020geom}. 
  Results "$\ddag$" are ran by searching the hyperparameters in the following ranges similar as Beaini et al.'s experimental setting \cite{beaini2021directional}: weight decay $\in [10^{-6}, 10^{-5}]$,
  learning rate $\in [10^{-5}, 10^{-4}]$,
  droupout ratio $\in [0.3, 0.5]$,
  aggreagators $\in\{$"mean-dir1-av", "mean-dir1-dx", "mean-dir1-av-dir1-dx"$\}$,
  net type $\in$ $\{$"complex", "simple"$\}$.
  For fair comparison, we use the same experimental setup as 
  \cite{pei2020geom},
  and report the average test accuracy over the same 10 fixed splits.}
  \label{table:real-res}
\end{table}

==> table_result_ablation.tex <==
% Table generated by Excel2LaTeX from sheet 'Results'
\begin{table*}[htbp]
% \hspace*{-1.2cm}
  \centering
  % \tiny
     \resizebox{1\hsize}{!}{
  \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccc|c|c|c|c|c|c|c|c|c}
    \toprule
   $\mathcal{R}(\mathcal{G})$%\tablefootnote{Neighour pruning} 
    & $\text{ATT}_\mathbf{e}$%\tablefootnote{Global directional aggregation} 
    & 
    $\mathbf{L}^{(\alpha, \gamma)}$%\tablefootnote{Parameterized random-walk Laplacian matrix} 
    & 
    chameleon & 
    squirrel & 
    actor  & 
    cornell & 
    wisconsin & 
    texas & 
    cora & 
    citeseer & 
    pubmed \\
    \midrule
    

    $\checkmark$ &       
    &      
    & 
    51.71 $\pm$ 1.23 &
    32.91 $\pm$ 2.26 & 
    35.24 $\pm$ 1.07 & 
    82.16 $\pm$ 5.94 &
    83.92 $\pm$ 3.59 & 
    78.38 $\pm$ 5.13 & 
    87.85 $\pm$ 1.02 & 
    74.50 $\pm$ 1.99 & 
    87.78 $\pm$ 0.44
    \\


    $\checkmark$ & 
    &
    $\checkmark$ &     
    
    51.91 $\pm$ 1.59 & 
    34.70 $\pm$ 1.02 &
    35.51 $\pm$ 0.74 &
    84.32 $\pm$ 4.15 & 
    84.12 $\pm$ 3.09 &
    78.65 $\pm$ 4.43 &
    87.83 $\pm$ 1.20 &
    76.18 $\pm$ 1.35 &
    87.93 $\pm$ 0.36 \\


    &       
    $\checkmark$ &      
    & 
    46.69 $\pm$ 1.98 &
    34.67 $\pm$ 0.10&
    29.63 $\pm$ 0.52 &
    60.27 $\pm$ 4.02 &
    54.51 $\pm$ 7.68 &
    60.81 $\pm$ 5.16 &
    87.95 $\pm$ 1.01 &
    76.31 $\pm$ 1.38 &
    87.90 $\pm$ 0.40 \\
    

    &       
    $\checkmark$ &      
    $\checkmark$ & 
    46.95 $\pm$ 2.50 &
    34.71 $\pm$ 1.02 &
    29.87 $\pm$ 0.60 &
    60.54 $\pm$ 0.40 &
    54.71 $\pm$ 5.68 &
    60.81 $\pm$ 4.87 &
    87.28 $\pm$ 1.53 &
    \textbf{76.41 $\pm$ 1.62} &
    87.88 $\pm$ 0.46 \\


    $\checkmark$ & 
    $\checkmark$ &       
    &     
    52.39 $\pm$ 2.08 &
    33.93 $\pm$ 1.86 &
    35.64 $\pm$ 0.10 &
    84.86 $\pm$ 5.12 &
    84.11 $\pm$ 2.69 &
    78.92 $\pm$ 5.57 &
    87.93 $\pm$ 0.99 &
    73.91 $\pm$ 1.62 &
    87.82 $\pm$ 0.30 \\


    $\checkmark$ & 
    $\checkmark$ &       
    $\checkmark$ &  
    \textbf{52.47 $\pm$ 1.44} &
    \textbf{34.82 $\pm$ 1.60} &
    \textbf{35.68 $\pm$ 1.20} &
    \textbf{85.14 $\pm$ 5.30} &
    \textbf{84.71 $\pm$ 3.59} &
    \textbf{79.46 $\pm$ 3.67} &
    \textbf{88.05 $\pm$ 1.09} &
    \textbf{76.41 $\pm$ 1.45} &
    \textbf{87.94 $\pm$ 0.48}
    \\

   \midrule
    &
    &
    &
    42.93 &
    30.03 &
    28.45 & 
    54.32 & 
    49.41 & 
    58.38 & 
    86.37 &
    74.32 &
    87.62  \\
   \bottomrule
   \end{tabular}%
   }
   \caption{Ablation study on 9 real-world datasets \cite{pei2020geom}. Cell with \checkmark means the component is applied to the DGAT model. The best test results are highlighted.}
   \label{tab:ablation_study}

\end{table*}

==> table_result_ablation_vertical.tex <==
\begin{table*}[htbp]
  %\left 
  \resizebox{1\hsize}{!}{
  \begin{tabular}{l|c|ccccc|c}
  \toprule
  $\mathcal{R}(\mathcal{G})$&
  &
  $\checkmark$&
  $\checkmark$&
  &
  &
  $\checkmark$&
  $\checkmark$

  \\

  $\text{ATT}_\mathbf{e}$&
  &
  &
  &
  $\checkmark$&
  $\checkmark$&
  $\checkmark$&
  $\checkmark$
  
  \\

  $\mathbf{L}^{(\alpha, \gamma)}$&
  &
  & 
  $\checkmark$&
  &
  $\checkmark$&
  &
  $\checkmark$
  
  \\

  \midrule
  chameleon&
  42.93&
  51.71 $\pm$ 1.23&
  51.91 $\pm$ 1.59&
  46.69 $\pm$ 1.98&
  46.95 $\pm$ 2.50&
  52.39 $\pm$ 2.08&
  \textbf{52.47 $\pm$ 1.44}
  
  \\

  squirrel&
  30.03&
  32.91 $\pm$ 2.26&
  34.70 $\pm$ 1.02&
  34.67 $\pm$ 0.10&
  34.71 $\pm$ 1.02&
  33.93 $\pm$ 1.86&
  \textbf{34.82 $\pm$ 1.60}
  
  \\

  actor&
  28.45&
  35.24 $\pm$ 1.07&
  35.51 $\pm$ 0.74&
  29.63 $\pm$ 0.52&
  29.87 $\pm$ 0.60&
  35.64 $\pm$ 0.10&
  \textbf{35.68 $\pm$ 1.20}
  
  \\

  cornell&
  54.32&
  82.16 $\pm$ 5.94&
  84.32 $\pm$ 4.15&
  60.27 $\pm$ 4.02&
  60.54 $\pm$ 0.40&
  84.86 $\pm$ 5.12&
  \textbf{85.14 $\pm$ 5.30}
  
  \\

  wisconsin&
  49.41&
  83.92 $\pm$ 3.59&
  84.12 $\pm$ 3.09&
  54.51 $\pm$ 7.68&
  54.71 $\pm$ 5.68&
  84.11 $\pm$ 2.69&
  \textbf{84.71 $\pm$ 3.59}
  
  \\


  texas&
  58.38&
  78.38 $\pm$ 5.13&
  78.65 $\pm$ 4.43&
  60.81 $\pm$ 5.16&
  60.81 $\pm$ 4.87&
  78.92 $\pm$ 5.57&
  \textbf{79.46 $\pm$ 3.67}
  
  \\

  cora&
  86.37&
  87.85 $\pm$ 1.02&
  87.83 $\pm$ 1.20&
  87.95 $\pm$ 1.01&
  87.28 $\pm$ 1.53&
  87.93 $\pm$ 0.99&
  \textbf{88.05 $\pm$ 1.09}
  
  \\

  citeseer&
  74.32&
  74.50 $\pm$ 1.99&
  76.18 $\pm$ 1.35&
  76.31 $\pm$ 1.38&
  \textbf{76.41 $\pm$ 1.62}&
  73.91 $\pm$ 1.62&
  \textbf{76.41 $\pm$ 1.45}
  
  \\

  pubmed&
  87.62&
  87.78 $\pm$ 0.44&
  87.93 $\pm$ 0.36&
  87.90 $\pm$ 0.40&
  87.88 $\pm$ 0.46&
  87.82 $\pm$ 0.30&
  \textbf{87.94 $\pm$ 0.48}
  
  \\
  \bottomrule
  \end{tabular}
  }
\caption{Ablation study on 9 real-world datasets \cite{pei2020geom}. Cell with \checkmark means the component is applied to the DGAT model.
The $\mathbf{L}^{(\alpha, \gamma)}$ means that the parameterized normalized Laplacian is used with optimal $\alpha$ and $\gamma$,
while unchecking $\mathbf{L}^{(\alpha, \gamma)}$ indicates that the default $\mathbf{L}^{(1, 1)} = \mathbf{L}_{\rw}$ is used.
The $\text{ATT}_\mathbf{e}$ is the global directional attention mechanism.
And $\mathcal{R}(\mathcal{G})$ is the graph re-wiring strategy.
DGAT without all component is just GAT,
whose results are reported from \cite{pei2020geom}.
The best test results are highlighted in \textbf{bold} format.}
\label{table:ablation_study_vertical}
\end{table*}

==> table_result_heter_ablation_dgcn.tex <==
\begin{table*}[ht]
\resizebox{1\hsize}{!}{
  \begin{tabular}{c|ccccccccc}
  \toprule
    Method&
    $\mathbf{P}^{(\alpha, \gamma)}$&
    $\mathcal{R}(\mathcal{G})$&
    roman-empire&
    amazon-ratings&
    minesweeper&
    tolokers&
    questions&
    squirrel filtered&
    chameleon filtered
    \\
    \midrule
    \multirow{1}[0]{*}
    &
    &
    &
    73.69 $\pm$ 0.74& 
    48.70 $\pm$ 0.63&
    89.75 $\pm$ 0.52&
    83.64 $\pm$ 0.67&
    76.09 $\pm$ 1.27&
    39.47 $\pm$ 1.47&
    40.89 $\pm$ 4.12
    
    \\

    \multirow{1}[0]{*}
    GCN&
    &
    $\checkmark$&
    74.50 $\pm$ 0.65&
    48.41 $\pm$ 0.44&
    89.93 $\pm$ 0.60&
    83.41 $\pm$ 0.94&
    77.27 $\pm$ 1.15&
    40.69 $\pm$ 2.13&
    43.96 $\pm$ 4.55
    
    \\

    \multirow{1}[0]{*}
    &
    $\checkmark$&
    $\checkmark$&
    &
    &
    &
    &
    &
    &
    
    
    \\
    
    \midrule

    \multirow{1}[0]{*}
    DP-GCN&
    $\checkmark$&
    &
    78.05 $\pm$ 0.49&
    49.49 $\pm$ 0.67&
    91.60 $\pm$ 0.62&
    83.83 $\pm$ 0.86&
    78.04 $\pm$ 0.91&
    43.31 $\pm$ 1.92&
    46.67 $\pm$ 3.56
    
    \\

    % \multirow{1}[0]{*}
    % &
    % $\checkmark$&
    % $\checkmark$&
    % &
    % &
    % &
    % &
    % &
    % &
    
    % \\


  \bottomrule
  \end{tabular}
  }
\caption{Ablation study of the parameterized diffusion with GCN (DP-GCN) on heterophily datasets proposed by \cite{platonov2023critical}.
A checkmark on $\mathbf{P}^{(\alpha, \gamma)}$ indicates the use of the parameterized normalized adjacency with optimal $\alpha$ and $\gamma$,
while an unchecked $\mathbf{P}^{(\alpha, \gamma)}$ denotes the use of the default $\mathbf{P}^{(1, 1)} = \mathbf{P}_{\rw}$.
The $\mathcal{R}(\mathcal{G})$ stands for the graph rewiring strategy and the best results are highlighted in \textbf{bold} format.
The results for GCN with $\mathcal{R}(\mathcal{G})$ comes from applying GCN on the rewired graph.
The rewiring technique is not applicable to DP-GCN, as DP-GCN assigns parameterized edge weights based on the original graph structure.
}
\label{tab:heter_ablation_dgcn}
\end{table*}

==> table_result_syn.tex <==
\begin{table}[htbp]
  \centering  
  \begin{tabular}{ccccc}
  \toprule
    $\mu$ 
    & GAT
    & GATv2
    & DGAT ($\gamma^{*}$)
    & DGAT ($\gamma^{-}$)
    \\
    \midrule
    0.0
    & 45.21
    & 48.66
    & \textbf{54.94 (0.1)}
    & 47.51 (0.7)
    \\

    0.1
    & 44.63
    & 50.65
    & \textbf{54.13 (0.3)}
    & 49.72 (0.9)
    \\
    
    0.2
    & 47.32
    & 54.46
    & \textbf{57.83 (0.3)}
    & 53.11 (1.0)
    \\
    
    0.3 
    & 56.59
    & 59.04
    &\textbf{64.33 (0.3)}
    & 59.37 (1.0) 
    \\
    
    0.4 
    & 63.21
    & 66.49
    & \textbf{73.54 (0.3)}
    & 66.71 (0.7)
    \\
    
    0.5
    & 74.14
    & 75.71
    &\textbf{82.95 (0.7)}
    & 78.81 (0.2) 
    \\
    
    0.6 
    & 83.96
    & 82.29
    & \textbf{90.56 (0.7)}
    & 88.30 (0.5)
    \\
    
    0.7
    & 89.33
    & 88.33
    & \textbf{96.00 (0.9)}
    & 94.85 (0.4)
    \\
    
    0.8
    & 94.92
    & 94.84
    & \textbf{98.67 (0.6)}
    & 97.84 (0.5)
    \\
    
    0.9
    & 98.62
    & 97.55
    & \textbf{99.58 (0.8)}
    & 98.21 (0.1)
    \\

  \bottomrule
  \end{tabular}

  \caption{Experimental results on synthetic graphs: average test accuracy (\%) with different homophily coefficients.
  The results are averaged over 5 random splits.
  The best results are in \textbf{bold} format. 
  For the DGAT model, we list the best and worst test runs (in the column DGAT ($\gamma^{*}$) and DGAT ($\gamma^{-}$) respectively) with different choices of  of $\gamma$ in the bracket, e.g. $54.94 (0.1)$ means that for $\gamma = 0.1$, the average test accuracy is $54.96\%$.}
  \label{table:syn_res}
\end{table}

==> table_result_vertical.tex <==
\begin{table}[htbp]
  %\left 
  \resizebox{1\hsize}{!}{
  \begin{tabular}{lccc}
  \toprule 
    Dataset ($\mathbf{H}_{\mathrm{node}}(\mathcal{G})$)
    & $\text{GAT}^{\dag}$
    & DGN  
    & DGAT
    %& $H_{\mathrm{node}}(\mathcal{G})$
    \\
    
    \midrule
    chameleon (0.25)
    & 42.93
    & 50.48 $\pm$ 1.26
    & \textbf{52.47 $\pm$ 1.44}
    %& 0.23
    \\

    squirrel (0.22)
    &30.03
    &\textbf{37.46 $\pm$ 1.28}
    & 34.82 $\pm$ 1.60
    %& 0.22
    \\

    actor (0.22)
    & 28.45
    & 35.47 $\pm$ 1.13
    & \textbf{35.68 $\pm$ 1.20}
    %& 0.22
    \\

    cornell (0.30)
    & 54.32
    & 77.03 $\pm$ 4.72
    & \textbf{85.14 $\pm$ 5.30}
    %& 0.30
    \\

    wisconsin (0.16)
    & 49.41
    & 82.75 $\pm$ 3.01
    & \textbf{84.71 $\pm$ 3.59}
    %& 0.21
    \\

    texas (0.06)
    &58.38
    &78.11 $\pm$ 4.90
    &\textbf{79.46 $\pm$ 3.67}
    %& 0.11
    \\

    cora (0.83)
    &86.37
    &84.69 $\pm$ 1.32
    &\textbf{88.05 $\pm$ 1.09}
    %&0.81
    \\

    citeseer (0.71)
    & 74.32
    & 73.87 $\pm$ 1.32
    & \textbf{76.41 $\pm$ 1.45}
    %& 0.74
    \\

    pubmed (0.79)
    & 87.62
    & 84.29 $\pm$ 0.61
    & \textbf{87.93 $\pm$0.48}
    %& 0.80
    \\
    % just change the previous table into vertical
    
  \bottomrule
  \end{tabular}
  }
  \caption{Benchmark with baselines on nine small real-world datasets.
  The best results are highlighted. 
  Results "$\dag$" are reported from \cite{pei2020geom}. 
  %Results "$\ddag$" are ran by searching the hyperparameters in the similar ranges as Beaini et al.'s experimental setting \cite{beaini2021directional}.
  For fair comparison, we use the same experimental setup as 
  \cite{pei2020geom},
  and report the average test accuracy over the same 10 fixed splits.}
  \label{table:real-res-vertical}
\end{table}
